Should we be going MAD? A Look at Multi-Agent Debate Strategies for LLMs

Recent advancements in large language models (LLMs) underscore their potential for responding to inquiries in various domains. However, ensuring that generative agents provide accurate and reliable answers remains an ongoing challenge. In this context, multi-agent debate (MAD) has emerged as a promising strategy for enhancing the truthfulness of LLMs. We benchmark a range of debating and prompting strategies to explore the trade-offs between cost, time, and accuracy. Importantly, we find that multi-agent debating systems, in their current form, do not reliably outperform other proposed prompting strategies, such as self-consistency and ensembling using multiple reasoning paths. However, when performing hyperparameter tuning, several MAD systems, such as Multi-Persona, perform better. This suggests that MAD protocols might not be inherently worse than other approaches, but that they are more sensitive to different hyperparameter settings and difficult to optimize. We build on these results to offer insights into improving debating strategies, such as adjusting agent agreement levels, which can significantly enhance performance and even surpass all other non-debate protocols we evaluated. We provide an open-source repository to the community with several state-of-the-art protocols together with evaluation scripts to benchmark across popular research datasets.

==> tables/full_results_table_old.tex <==
\small
% \pagenumbering{gobble}
\begin{landscape}

\begin{longtable}{lllllllllll}
\toprule

System Name & Debate Prompt & Agent prompt & Debate Config & Agents &
\multicolumn{2}{c}{MedQA} & \multicolumn{2}{c}{MMLU} & \multicolumn{2}{c}{PubMedQA} \\
 &   &    &    &   & Score & Cost \$ & Score & Cost \$ & Score & Cost \$ \\
\midrule
\endhead
\midrule
\multicolumn{10}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
Single Agent & - & CoT &  & GPT3.5 & 0.51 & 4.46 & 0.65 & 3.82 & 0.77 & 1.75 \\
Single Agent & - & CoT &  & GPT3.5 & 0.49 & 4.46 & 0.67 & 0.11 & 0.74 & 1.75 \\
Single Agent & - & CoT &  & PaLM & 0.14 & 1.28 & 0.30 & 0.03 & 0.42 & 0.50 \\
Single Agent & - & CoT &  & PaLM & 0.17 & 1.27 & 0.33 & 0.03 & 0.38 & 0.50 \\
Single Agent & - & FS &  & GPT3.5 & 0.53 & 4.46 & 0.70 & 0.11 & 0.71 & 1.75 \\
Single Agent & - & FS &  & PaLM & 0.46 & 1.27 & 0.50 & 0.03 & 0.75 & 0.50 \\
Single Agent & - & FS+EG &  & GPT3.5 & 0.54 & 6.37 & 0.80 & 0.11 & 0.70 & 2.61 \\
Single Agent & - & FS+EG &  & PaLM & 0.47 & 1.91 & 0.70 & 0.03 & 0.65 & 0.86 \\
Single Agent & - & FS-CoT &  & GPT3.5 & 0.56 & 6.37 & 0.70 & 0.15 & 0.79 & 2.60 \\
Single Agent & - & FS-CoT &  & PaLM & 0.49 & 1.91 & 0.63 & 0.04 & 0.71 & 0.86 \\
Single Agent & - & SIMPLE &  & GPT3.5 & 0.52 & 4.46 & 0.73 & 0.11 & 0.71 & 1.75 \\
Single Agent & - & SIMPLE &  & PaLM & 0.46 & 1.27 & 0.68 & 1.09 & 0.76 & 0.50 \\
Single Agent & - & SPP & SPP Synergy & GPT3.5 & 0.53 & 6.38 & 0.70 & 0.04 & 0.69 & 2.55 \\
ChatEval & CE MAD & CoT & 3 rounds, one by one & GPT3.5 & 0.53 & 34.81 & 0.74 & 3.06 & 0.76 & 12.60 \\
ChatEval & CE MAD & CoT & 2 rounds, simultaneous talk & GPT3.5 & 0.54 & 19.90 & 0.79 & 1.76 & 0.74 & 7.27 \\
ChatEval & CE MAD & CoT & 3 rounds, simultaneous talk with summarizer & GPT3.5 & 0.55 & 36.78 & 0.78 & 3.46 & 0.77 & 14.01 \\
ChatEval & CE MAD & CoT & 2 rounds, one by one & GPT3.5 & 0.55 & 20.55 & 0.77 & 1.82 & 0.76 & 7.64 \\
ChatEval & CE MAD & CoT & 2 rounds, simultaneous talk with summarizer & GPT3.5 & 0.55 & 22.58 & 0.73 & 2.16 & 0.72 & 8.76 \\
ChatEval & CE MAD & CoT & 3 rounds, simultaneous talk & GPT3.5 & 0.57 & 33.26 & 0.76 & 2.93 & 0.77 & 12.14 \\
Ensemble Refinement & ER MAD & FS & reasoning=3, aggregation=9 & GPT3.5 & 0.53 & 53.57 & 0.70 & 5.17 & 0.72 & 21.00 \\
Ensemble Refinement & ER MAD & FS & reasoning=3, aggregation=1 & GPT3.5 & 0.53 & 17.83 & 0.69 & 1.72 & 0.72 & 7.00 \\
Ensemble Refinement & ER MAD & FS & self consistency: reasoning=5 & GPT3.5 & 0.53 & 22.28 & 0.73 & 2.15 & 0.70 & 8.75 \\
Ensemble Refinement & ER MAD & FS & self consistency: reasoning=5 & PaLM & 0.46 & 6.36 & 0.70 & 0.62 & 0.76 & 2.50 \\
Ensemble Refinement & ER MAD & FS+EG & reasoning=3, aggregation=9 & GPT3.5 & 0.54 & 76.60 & 0.72 & 5.21 & 0.74 & 33.21 \\
Ensemble Refinement & ER MAD & FS+EG & reasoning=3, aggregation=1 & GPT3.5 & 0.54 & 25.50 & 0.72 & 1.73 & 0.76 & 10.64 \\
Ensemble Refinement & ER MAD & FS+EG & self consistency: reasoning=5 & GPT3.5 & 0.54 & 31.86 & 0.72 & 2.15 & 0.71 & 13.04 \\
Ensemble Refinement & ER MAD & FS+EG & self consistency: reasoning=5 & PaLM & 0.47 & 9.57 & 0.69 & 0.62 & 0.71 & 4.30 \\
Ensemble Refinement & ER MAD CoT & CoT & reasoning=3, aggregation=1 & GPT3.5 & 0.54 & 19.53 & 0.72 & 1.82 & 0.77 & 7.54 \\
Ensemble Refinement & ER MAD CoT & CoT & self consistency: reasoning=5 & GPT3.5 & 0.54 & 22.28 & 0.70 & 2.15 & 0.78 & 8.75 \\
Ensemble Refinement & ER MAD CoT & CoT & reasoning=3, aggregation=9 & GPT3.5 & 0.55 & 69.00 & 0.67 & 1.50 & 0.75 & 25.60 \\
Ensemble Refinement & ER MAD CoT & CoT & self consistency: reasoning=5 & PaLM & 0.17 & 6.36 & 0.58 & 0.62 & 0.38 & 2.50 \\
Ensemble Refinement & ER MAD CoT & FS-CoT & self consistency: reasoning=5 & GPT3.5 & 0.59 & 31.84 & 0.85 & 3.08 & 0.79 & 13.01 \\
Ensemble Refinement & ER MAD CoT & FS-CoT & reasoning=3, aggregation=9 & GPT3.5 & 0.60 & 83.03 & 0.83 & 8.00 & 0.78 & 37.22 \\
Ensemble Refinement & ER MAD CoT & FS-CoT & reasoning=3, aggregation=1 & GPT3.5 & 0.60 & 26.18 & 0.82 & 2.51 & 0.77 & 11.07 \\
Ensemble Refinement & ER MAD CoT & FS-CoT & self consistency: reasoning=5 & PaLM & 0.52 & 9.56 & 0.69 & 0.92 & 0.72 & 4.29 \\
Multi-Persona & MP MAD & ANGEL+DEVIL & 3 rounds max & GPT3.5 & 0.49 & 15.15 & 0.71 & 1.50 & 0.71 & 8.82 \\
Multi-Persona & MP MAD & ANGEL+DEVIL & 4 rounds max & GPT3.5 & 0.50 & 15.08 & 0.70 & 1.45 & 0.69 & 10.00 \\
Multi-Persona & MP MAD & ANGEL+DEVIL & 2 rounds max & GPT3.5 & 0.51 & 14.41 & 0.67 & 1.39 & 0.71 & 7.11 \\
Society of Mind & SoM MAD & CoT & 2 agents, 2 rounds, summarized answers & GPT3.5 & 0.57 & 17.83 & 0.72 & 1.72 & 0.73 & 7.00 \\
Society of Mind & SoM MAD & CoT & 2 agents, 2 rounds & GPT3.5 & 0.58 & 18.05 & 0.67 & 1.72 & 0.76 & 7.00 \\
Society of Mind & SoM MAD & CoT & 3 agents, 3 rounds & GPT3.5 & 0.59 & 41.94 & 0.71 & 3.88 & 0.76 & 15.80 \\
Society of Mind & SoM MAD & CoT & 2 agents, 3 rounds & GPT3.5 & 0.59 & 26.94 & 0.67 & 2.58 & 0.76 & 10.50 \\
Society of Mind & SoM MAD & CoT & 4 agents, 2 rounds, summarized answers & GPT3.5 & 0.59 & 35.65 & 0.72 & 3.44 & 0.77 & 14.00 \\
Society of Mind & SoM MAD & CoT & 3 agents, 2 rounds, summarized answers & GPT3.5 & 0.59 & 26.74 & 0.70 & 2.58 & 0.76 & 10.50 \\
Society of Mind & SoM MAD & CoT & 4 agents, 2 rounds & GPT3.5 & 0.60 & 38.96 & 0.71 & 3.47 & 0.74 & 14.02 \\
Society of Mind & SoM MAD & CoT & 2 agents, 3 rounds, summarized answers & GPT3.5 & 0.60 & 26.74 & 0.72 & 2.58 & 0.74 & 10.51 \\
Society of Mind & SoM MAD & CoT & 4 agents, 3 rounds & GPT3.5 & 0.61 & 58.52 & 0.71 & 5.20 & 0.74 & 21.40 \\
Society of Mind & SoM MAD & CoT & 3 agents, 2 rounds & GPT3.5 & 0.61 & 28.04 & 0.74 & 2.59 & 0.75 & 10.50 \\
Society of Mind & SoM MAD & CoT & 4 agents, 3 rounds, summarized answers & GPT3.5 & 0.61 & 53.48 & 0.72 & 5.17 & 0.72 & 21.01 \\
Society of Mind & SoM MAD & CoT & 3 agents, 3 rounds, summarized answers & GPT3.5 & 0.61 & 40.11 & 0.75 & 3.87 & 0.72 & 15.75 \\

\caption{Complete table of experiment configurations}\label{app:tab:full-results-table}

\end{longtable}
\end{landscape}


